OPA-3D: Occlusion-Aware Pixel-Wise Aggregation for Monocular 3D Object Detection

Despite monocular 3D object detection having recently made a significant leap forward thanks to the use of pre-trained depth estimators for pseudo-LiDAR recovery, such two-stage methods typically suffer from overfitting and are incapable of explicitly encapsulating the geometric relation between depth and object bounding box. To overcome this limitation, we instead propose OPA-3D, a single-stage, end-to-end, Occlusion-Aware Pixel-Wise Aggregation network that to jointly estimate dense scene depth with depth-bounding box residuals and object bounding boxes, allowing a two-stream detection of 3D objects, leading to significantly more robust detections. Thereby, the geometry stream denoted as the Geometry Stream, combines visible depth and depth-bounding box residuals to recover the object bounding box via explicit occlusion-aware optimization. In addition, a bounding box based geometry projection scheme is employed in an effort to enhance distance perception. The second stream, named as the Context Stream, directly regresses 3D object location and size. This novel two-stream representation further enables us to enforce cross-stream consistency terms which aligns the outputs of both streams, improving the overall performance. Extensive experiments on the public benchmark demonstrate that OPA-3D outperforms state-of-the-art methods on the main Car category, whilst keeping a real-time inference speed. We plan to release all codes and trained models soon.

==> sections/Tab1.tex <==
\begin{table*}[t]
\centering

\caption{{Comparison with state-of-the-art methods of the \textit{car} category on KITTI-3D.}
}
\begin{threeparttable}

\begin{tabular}{c|c|ccc|ccc|c}
\hline
\multirow{2}{*}{Method}  & \multirow{2}{*}{Extra Data}  & \multicolumn{3}{c|}{ Test Split } &  \multicolumn{3}{c|}{ Validation Split } & Time\\
\cline{3-9}
& & Mod. & Easy & Hard & Mod. & Easy & Hard & (sec) \\
\hline
ROI-10D~\cite{roi10d} & None & 2.02 & 4.32 & 1.46 & 6.63 & 9.61 & 6.29 & 0.2 \\
MonoPair~\cite{chen2020monopair} & None & 9.99 & 13.04 & 8.65 & 12.30 & 16.28 & 10.42 & 0.057 \\
DLE~\cite{ma2021delving} & None & 12.26 & 17.23 & 10.29 & 13.66 & 17.45 & 11.68 & 0.040 \\
GUP-Net~\cite{gupnet} & None & 15.02 & 22.26 & 13.12 &	16.46 & 22.76 &	13.72 & 0.034 \\
Monocon~\cite{monocon} & None & 16.46 & 22.50 &	13.95 & 19.01 & \textbf{26.33} & 15.98 & 0.026 \\
\hline
DD3D~\cite{DD3D} & Depth$^{*}$ & \underline{16.87} & \underline{23.19} & \textbf{14.36} & (16.92) & - & - & - \\ 
\hline
D4LCN~\cite{D4LCN} & Depth & 11.72 & 16.65 & 9.51 & - &	- & - & 0.20 \\
CaDNN~\cite{cadnn} & LiDAR & 13.41 & 19.17  & 11.46 & 16.31 & 23.57 & 13.84 & 0.63 \\ 
AutoShape~\cite{liu2021autoshape} & CAD Model & 14.17 & 22.47 & 11.36 & 14.65 & 20.09 & 12.07 & 0.050 \\
MonoDistill~\cite{chong2022monodistill} & LiDAR & 16.03 & 22.97 & 13.60 & 18.47 & 24.31 & 15.76 & 0.040 \\
Ours & Depth & \textbf{17.05} & \textbf{24.60} & \underline{14.25} & \textbf{19.40} & \underline{24.97} & \textbf{16.59} & 0.040 \\

\hline
\end{tabular}

\footnotesize
Overall best results are in bold and the second best results are underlined.  
Methods are ranked according to the moderate AP for the IoU metric at a 0.7 threshold as given in the KITTI-3D benchmark.
Note that on the test split DD3D utilizes deeper V2-99~\cite{v299} instead of DLA-34 as the feature extractor, and also pre-trains the network on the unreleased large-scale DD3D15M dataset, while OPA-3D only uses DLA-34 and pretrains on the clean split of KITTI-Depth dataset~\cite{DD3D} for fair comparison with the SOTA. 
On the validation split, we report the result of DD3D with DLA-34~\cite{dla34} as the backbone.

\end{threeparttable}

\label{tab:kitti_test_car}
\end{table*}

==> sections/Tab2.tex <==
\begin{table*}[t]
\centering
\caption{{Comparison with state-of-the-art methods of the \textit{pedestrian} and \textit{cyclist} on KITTI-3D testing split. AP for the IoU metric at a 0.7 threshold is reported.}
}
\begin{threeparttable}

\begin{tabular}{c|c|ccc|ccc|c}
\hline
\multirow{2}{*}{Method}  & \multirow{2}{*}{Extra Data}  & \multicolumn{3}{c|}{ Pedestrian } &  \multicolumn{3}{c|}{ Cyclist } & Time\\
\cline{3-9}
& & Mod. & Easy & Hard & Mod. & Easy & Hard & (sec) \\
\hline
MonoPair~\cite{chen2020monopair} & None & 6.68 & 10.02 & 5.53 & 2.12 & 3.79 & 1.83 & 0.057 \\
DLE~\cite{ma2021delving} & None & 6.55 & 9.64 & 5.44 & 2.66 & 4.59 & 2.45 & 0.040 \\
GUP-Net~\cite{gupnet} & None & 9.76 & 14.95 & 8.41 & \underline{3.21} & 5.58 &	2.66 & 0.034 \\
Monocon~\cite{monocon} & None & 8.41 & 13.10 &	6.94 & 1.92 & 2.80 & 1.55 & 0.026 \\
\hline
DD3D~\cite{DD3D} & Depth$^{*}$ & \textbf{11.04}& \textbf{16.64} & \textbf{9.38} & \textbf{4.79} &  \textbf{7.52} & \textbf{4.22} & - \\ 
\hline
D4LCN~\cite{D4LCN} & Depth & 3.42 & 4.55 & 2.83 & 1.67 & 2.45 & 1.36 & 0.20 \\
CaDNN~\cite{cadnn} & LiDAR & 8.14 & 12.87  & 6.76 & 3.41 & \underline{7.00} & \underline{3.30} & 0.63 \\ 
Ours & Depth & \underline{10.49} & \underline{15.65} & \underline{8.80} & 3.45 & 5.16 & 2.86 & 0.040 \\

\hline
\end{tabular}
\footnotesize
Overall best results are in bold and the second best results are underlined. 
\end{threeparttable}

\label{tab:kitti_test_other}
\end{table*}

==> sections/Tab3.tex <==
\begin{table}[t]
\centering
\caption{{Ablation study of the \textit{car} category on KITTI-3D validation split.}
}
\begin{threeparttable}

\begin{tabular}{c|c|c|c|ccc|ccc}
\hline
\multirow{2}{*}{Stage}  & \multicolumn{3}{c|}{ Geometry Stream } & \multicolumn{3}{c|}{3D $AP_{IoU \geq 0.7}$ } & \multicolumn{3}{c}{BEV $AP_{IoU \geq 0.7}$ }\\
\cline{2-4}
\cline{5-10}
& Pretrained & $\ll_{C-G}$ & $\ll_{BPC}$ & Mod. & Easy & Hard & Mod. & Easy & Hard\\
\hline
A & & & & 15.76 & 22.01 & 13.11 & 22.43 & 30.87 & 19.32 \\
\hline
B1 & & \checkmark & & 18.10 & 24.81 & 15.27 & 24.66 & 32.58& 21.38 \\
B2 & \checkmark  & \checkmark & & 18.71 & 26.44 & 15.64 &25.16 & 34.84 & 20.79 \\
\hline
C & & & \checkmark & 18.00 & 24.51 & 15.15 & 24.60 & 32.05 & 21.27\\
\hline
D & \checkmark & \checkmark & \checkmark & 19.40 & 24.97 & 16.59 & 25.51 & 33.80 & 22.13 \\

\hline
\end{tabular}
\footnotesize
We ablate the proposed $\ll_{C-G}$ and $\ll_{BPC}$ in the geometry stream, and verify the effect of pre-training. 
\end{threeparttable}

\label{tab:kitti_ablation}
\end{table}

==> sections/Tab4.tex <==
\begin{table*}[t]
\centering
\caption{{Comparison with state-of-the-art methods of the \textit{car} category on the KITTI-3D validation split.}
}
\begin{threeparttable}

\begin{tabular}{c|c|ccc|ccc|c}
\shline
\multirow{2}{*}{Method}  & \multirow{2}{*}{Extra Data}  & \multicolumn{3}{c|}{ 3D $AP_{IoU \geq 0.7}$ } &  \multicolumn{3}{c|}{ BEV $ AP_{IoU \geq 0.7}$ } & Time\\
\cline{3-9}
& & Mod. & Easy & Hard & Mod. & Easy & Hard & (sec) \\
\hline
MonoPair~\cite{chen2020monopair} & None & 12.30 & 16.28 & 10.42 & 18.17 & 24.12 & 15.76 & 0.057 \\
DLE~\cite{ma2021delving} & None & 13.66 & 17.45 & 11.68 & 19.33 & 24.97 & 17.01 & 0.040 \\
GUP-Net~\cite{gupnet} & None & 16.46 & 22.76 & 13.72 &	22.94 & 31.07 &	19.75 & 0.034 \\
\hline
MonoDistill~\cite{chong2022monodistill} & LiDAR & 18.47 & 24.31 & 15.76 & 25.40 & 33.09 & 22.16 & 0.040 \\
CaDNN~\cite{cadnn} & LiDAR & 16.31 & 23.57  & 13.84 & - & - & - & 0.63 \\ 
DD3D~\cite{DD3D} & Depth$^{*}$ & 16.92 & - & - & 24.77 & - & -& -\\
Ours & Depth & 19.40 & 24.97 & 16.59 & 25.51 & 33.80 & 22.13 & 0.040 \\

\shline
\end{tabular}
\footnotesize
Overall best results are in bold and the second best results are underlined.  
Methods are ranked according to the mediate 3D IoU results like in the KITTI-3D benchmark.
\end{threeparttable}

\label{tab:kitti_val}
\end{table*}
